Empathosphere: Promoting Constructive Communication in Ad-hoc Virtual Teams through Perspective-taking Spaces

When members of ad-hoc virtual teams need to collectively ideate or deliberate, they often fail to engage with each others' perspectives in a constructive manner. At best, this leads to sub-optimal outcomes and, at worst, it can cause conflicts that lead to teams not wanting to continue working together. Prior work has attempted to facilitate constructive communication by highlighting problematic communication patterns and nudging teams to alter interaction norms. However, these approaches achieve limited success because they fail to acknowledge two social barriers: (1) it is hard to reset team norms mid-interaction, and (2) corrective nudges have limited utility unless team members believe it is safe to voice their opinion and that their opinion will be heard. This paper introduces Empathosphere, a chat-embedded intervention to mitigate these barriers and foster constructive communication in teams. To mitigate the first barrier, Empathosphere leverages the benefits of "experimental spaces" in dampening existing norms and creating a climate conducive to change. To mitigate the second barrier, Empathosphere harnesses the benefits of perspective-taking to cultivate a group climate that promotes a norm of members speaking up and engaging with each other. Empathosphere achieves this by orchestrating authentic socio-emotional exchanges designed to induce perspective-taking. A controlled study (N=110) compared Empathosphere to an alternate intervention strategy of prompting teams to reflect on their team experience. We found that Empathosphere led to higher work satisfaction, encouraged more open communication and feedback within teams, and boosted teams' desire to continue working together. This work demonstrates that ``experimental spaces,'' particularly those that integrate methods of encouraging perspective-taking, can be a powerful means of improving communication in virtual teams.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> sections-old/00_abstract.tex <==
Ad-hoc virtual teams struggle to engage in productive dialogue - when members need to work together to ideate or deliberate, they often fail to engage with each others' perspectives in a constructive manner. At best, this leads to sub-optimal outcomes and, at worst, it can cause conflicts that lead to teams not wanting to continue working together. Prior work has attempted to facilitate constructive communication by highlighting problematic communication patterns and making suggestions on how teams should alter their interaction norms. However, these interventions have had limited success because they fail to acknowledge two social barriers: (1) it is hard to reset team norms mid-interaction, and (2) corrective instructions will have limited utility unless team members believe it is safe to voice their opinion and that their opinion will be heard. This paper introduces \sys{}, a chat-embedded intervention designed to mitigate these barriers and foster constructive communication in teams. To mitigate the first barrier, \sys{} leverages the known benefits of ``experimental spaces'' in dampening existing norms and creating a climate conducive to change. \sys{} instantiates this ``space'' as a separate communication channel in a team's workspace. To mitigate the second barrier, \sys{} harnesses the benefits of perspective-taking to cultivate a group climate that promotes a norm of group members speaking up and engaging with each other. \sys{} achieves this by orchestrating authentic socio-emotional exchanges designed to induce perspective-taking. A controlled study ($N=110$) with ad-hoc groups recruited from Amazon Mechanical Turk compared \sys{} to an alternate intervention strategy of prompting teams to reflect on their team experience. Results revealed that groups randomly assigned to experience \sys{} reported higher work satisfaction, exhibited more open communication and feedback, and expressed greater desire to continue working together. This research demonstrates that ``experimental spaces,'' particularly those that integrate established methods of encouraging perspective-taking, can be a powerful means of increasing the viability and effectiveness of computer-mediated teams.





==> sections-old/01_introduction.tex <==
Virtual teams, convened on online platforms, have demonstrated the potential to accomplish complex tasks, but are currently limited in their ability to collaborate effectively. Virtual teams have tackled problems ranging from open design~\cite{Salehi2018-vt} to software development~\cite{Valentine2017-qu} and research~\cite{vaish2017crowd}. 
% When tasks can be decomposed into fragments and members' roles can be well defined, virtual teams thrive but when team members need to come together, interact, co-ideate, and deliberate, virtual teams are vulnerable to conflict and misunderstanding. 
However, the reliance on computer-mediated communication can make it more difficult to establish communication norms that promote sharing and engaging with each others' ideas and perspectives. 
Computer mediation lowers socioemotional communication and virtual teams are less cohesive than collocated teams, exhibiting lower trust and shared identity~\cite{hinds2003out}. As a result, team members are less likely to speak up and openly express their perspectives~\cite{morrison2011speaking}. 
Furthermore, even when team members express their perspectives, these are likely to be ignored by other members, triggering conflict and threatening the team's performance and sustainability~\cite{hinds2003out}. 

Thus, virtual teams can be even more effective at collaboration if they can use the diverse perspectives and unique expertise of individual members. To do so, team members need to learn to communicate effectively in an open and respectful manner, integrating everyone's perspectives. This problem is even more challenging for teams where team membership often changes, as is common in virtual teams~\cite{Salehi2018-vt, Valentine2017-qu}, For such high-turnover teams, developing effective communication and accommodating new team members is an ongoing challenge. This paper introduces a new system to foster open and ... communication, by creating spaces...

Prior work has attributed the difficulty of establishing healthy communication to the low levels of information richness, lack of social cues, context, and shared emotion in computer-mediated teams~\cite{Hinds2003-ky}. In response to this, researchers have developed new communication channels~\cite{hassib2017heartchat, buschek2015there,lee2006using,wang2004communicating} to increase information richness and novel sociometric feedback mechanisms~\cite{viegas1999chat,tat2002visualising,tat2006crystalchat} to improve social awareness. While these systems enhance awareness about suboptimal behaviors and provide mediums for team members to be more expressive, in practice, several social and psychological barriers prevent team members from using these mechanisms to proactively shape communication norms. Despite the benefits of open and frank communication, team members often do not speak up. When new members are learning to work together in a team, an uncertainty about group norms and potential consequences of speaking up, coupled with lower shared identity, can cause members to view expressing disagreement, voicing concerns, or asking questions as risky. They may believe that their inputs will not be taken seriously~\cite{morrison2011speaking}. All of which discourages team members from speaking up~\cite{morrison2011speaking}. This often leads to unanticipated outcomes: prior work found that when teams were alerted about low group-level agreement as measured in their chat messages, team members responded by passively expressing agreement with each other which led to lower quality work~\cite{Leshed2009-eq}. Such a ``climate of silence''~\cite{Morrison2000-uu} can undermine team performance~\cite{perlow2003silence, argyris1991teaching}.

We leverage the construct of ``spaces''~\cite{zietsma2010institutional, furnari2014interstitial} to foster open and respectful communication by mitigating some of the associated social and psychological barriers. Spaces are social settings separated by physical, temporal or symbolic boundaries from everyday work within which the salience of existing norms and interaction patterns diminishes. This creates an environment conducive to risky and counternormative behaviors that can catalyze the emergence of new dynamics~\cite{Lee2020-zn, bucher2016interplay, furnari2014interstitial, zietsma2010institutional}. This paper introduces a system that leverages spaces in the context of online team communication environments to improve team communication.

 \begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/interfaces.pdf}
    \caption{We introduce a "space" within a chat-based collaboration environment (A) as a temporally and spatially demarcated meta-channel within which team members engage in an intervention aimed at improving perspective-taking and fostering open and respectful communication (B).}
    \label{fig:space}
\end{figure}

We instantiate our "space" as a temporally and spatially demarcated meta-channel within a chat-based collaboration environment (Fig. \ref{fig:space}). We designed and deployed an intervention, within this space, to support processes known to improve perspective-taking while maintaining the ambiguity and anonymity necessary to promote authentic expression. Drawing attention to others' emotions and affective states- \textit{attention modulation}- can increase perspective-taking~\cite{zaki2014empathy,curran2019understanding}. To support this process, we privately elicit how team members actually feel about working with their group and provide the group feedback about the aggregate group climate without revealing individual responses. We also ask each member, in private, to guess how other members might be feeling, to nudge them to direct their attention towards others in the team. Perspective-taking is also regulated by \textit{appraisal} or an individual's evaluation of the authenticity and intensity of others' emotions~\cite{zaki2014empathy}. Emotions expressed privately in the ``space'' are more authentic and uninhibited than those expressed in the chat. So, team members are more likely to recognize potential grievances and act on them when they are confronted with them within the space. Taken together, we expect our intervention to improve perspective-taking and foster open communication. We expect these positive dynamics will also improve team satisfaction and team viability- team members' desire to continue working together.

To test the efficacy of our intervention, we conducted a controlled-study ($N=110$ in 24 teams) where we compared the benefits of our intervention against the benefits of injecting a reflective pause in team communication. In both conditions, participants recruited from Amazon Mechanical Turk worked synchronously on a decision-making task, in teams of 4-6 via our chat-based collaboration system. Based on the condition assigned to the team, the system injected either the intervention or a reflective pause in the teamwork session. Through surveys at the end of the study, we probed participants for team viability (whether they would consider working with their team gain), perceived conflict, willingness to exchange feedback with team members, and their satisfaction with their team's final solution. 

We found that compared to the control condition, participants in the intervention condition judged their teams to be significantly more viable while we found no significant differences in perceived levels of task and relationship conflict. Furthermore, we find that participants in the intervention condition were approximately 25.4\% more likely to be willing to provide feedback to teammates than in the control condition (p=0, t(45)=45). Correspondingly a marginally larger fraction of participants in the intervention condition was willing to receive feedback from teammates. Participants in the intervention condition also reported being more significantly more satisfied with their team's final solution than participants in the control condition. Talk about language use differences.

Our findings suggest that embedding computationally-mediated interventions within collaboration environments are a powerful tool in helping teams establish positive interaction norms. Our experiments focused on initial interactions of newly convened remote teams, collaborating over short durations, however, fostering positive interaction dynamics isn't just a one-time process- even long-standing teams are often reconfigured and so, team members have to frequently learn to work with new people. Repeated deployment of the intervention whenever teams experience changes in membership could help teams adapt. While we specifically studied virtual teams, collocated teams also struggle with fostering an environment of open and respectful communication- they could also benefit from computationally-mediated interventions when initially learning to work together.
% When running studies on AMT, the short time frame of the experiment combined with their expectation of future separation causes participants to focus on the completion of the task, while disincentivizing efforts to form cohesive team norms that would only benefit them if they continued working together~\cite{Bradley2003-aa}. Despite this, we were able to observe effects of our intervention 

==> sections-old/01_introductionv1.tex <==
% Teams as an organizational structure benefit from diverse perspectives and opinions of its members. They can lead to improved ideas, better decisions. But just the existence of diverse perspectives in insufficient, you need people to engage with each others diverse perspectives. Conflicting ideas or opinions need to be expressed and the team should be able to handle the conflict effectively.

% Current collaboration environments lack affordances to support these meta-level processes. 

Respectful, open, and critical communication is crucial for effective collaboration. %This is good
Open communication of ideas, suggestions, opinions, and issues, can help uncover new solutions~\cite{Menold2019-wc}, improve decision making \wesley{citation here as well?}, facilitate team learning~\cite{morrison2011speaking, Morrison2000-uu}, and help identify and address problems \wesley{citation here as well?}. However merely expressing opinions is not enough- to achieve improved outcomes, team members must also engage with others' perspectives, foster inclusivity, and affirm others~\cite{Salehi2018-vt, Carmeli2015-qv, Hoever2012-hn}. The diverse perspectives and unique expertise of individual members make teams potent and so, for teams to be effective it is crucial that team-members both speak up, expressing their perspectives, and that they listen to and engage with others' perspectives, in a respectful manner~\cite{morrison2011speaking}. Failure to take everyone's opinions into account can trigger negative emotions causing members to get angry and distressed~\cite{Jung2015-px}. Negative emotions also have a tendency to escalate and spiral out of control~\cite{Jung2015-px}. Absence of healthy communication can thus cause interpersonal friction and ultimately, undermine team performance [cite from voice paper]. Computer-mediated teams are especially vulnerable. Low levels of information richness, lack of social cues, context, and shared emotion can make it challenging to establish healthy communication patterns in computer-mediated teams- they are prone to misunderstanding and conflicts~\cite{Hinds2003-ky}.

To improve communication patterns in computer-mediated teams, researchers have designed systems that attempt to make existing communication dynamics in a team, visible, with the hope that it will help teams identify suboptimal group dynamics and move towards more positive communication patterns. This includes novel tools to measure behavioral metrics like agreement, engagement, turn-taking, language use, and content focus as well as novel mechanisms to communicate sociometric feedback to teams.~\cite{Kim2012-jv,Leshed2009-eq,Tausczik2013-br, Leshed2007-up}. Some tools go beyond making extant behaviors salient and also make specific recommendations on how teams should alter their practices to move them closer to desired behaviors~\cite{Tausczik2013-br}. However, these systems don't capture true emotional states of teams- they only capture measurable proxies for underlying emotional states. Synchronicity and positive sentiment in chat messages might be used as a proxy for actual agreement between team members~\cite{Leshed2009-eq}. Since there is often a disconnect between how team members feel and what they are comfortable expressing~\cite{morrison2011speaking}, prescriptive interventions, based on measurable proxies, often fail to prompt team members to confront underlying issues and instead, team members merely seek to achieve desirable levels of surface-level proxies: prior work found that visualizing group-level agreement prompted team members to passively express agreement with each other while actually resulting in lower quality work~\cite{Leshed2009-eq}. This hints at teams adopting an avoidance approach~\cite{kankanhalli2006conflict} to conflict resolution which leaves conflict unresolved and hinders teamwork. Despite the benefits of open and frank communication, team members often do not speak up. They may view expressing disagreement, voicing concerns, or asking questions as risky or they may believe that their inputs will not be taken seriously~\cite{morrison2011speaking}. These beliefs about speaking up are shaped by the interaction history of the team~\cite{morrison2011speaking}. For newly convened teams, an uncertainty about group norms and potential consequences of speaking up could discourage employees from speaking up. For teams that have an interaction history, past instances of group members receiving flak for speaking up can result in a similar group climate. Relatedly, team members who do not strongly identify with their team or who are unsatisfied with their team, might think speaking up is futile~\cite{morrison2011speaking}. Regardless of the cause, a ``climate of silence''~\cite{Morrison2000-uu} can undermine team performance~\cite{perlow2003silence, argyris1991teaching}. How might we promote more constructive communication behaviors that team members view as risky? \wesley{I think this paragraph grounds super well in the previous literature and covers a lot of important motivations for the work. Maybe having the most important several being \textbf{BOLD} or list 1) 2) 3)? I kinda feel like there's too much information to process here.}

The critical insight in our work is leveraging the organizational science of ``spaces''~\cite{furnari2014interstitial}. Spaces are bounded social settings that facilitate counternormative behaviors~\cite{Lee2020-zn, bucher2016interplay, furnari2014interstitial, zietsma2010institutional}. For example, retreat? Spaces facilitate more open and respectful communication, while recognizing the social and psychological barriers preventing it. This paper introduces a system that leverages spaces in the context of online team communication environments to improve team communication.


Spaces are social settings separated by physical, temporal or symbolic boundaries from everyday work within which the salience of existing norms and interaction patterns diminishes. This creates an environment conducive to risky and counternormative behaviors that can catalyze the emergence of new dynamics~\cite{Lee2020-zn, bucher2016interplay, furnari2014interstitial, zietsma2010institutional}. [Example of a space - office party/retreat]. Spaces provide a lightweight way to reset communication patterns. We attempt to imagine what such a space might look like in the context of online team communication environments and how we might use such a space to develop interventions to improve team communication.

We instantiate our "space" as a temporally and spatially demarcated meta-channel within a chat-based collaboration environment. We design an intervention that we deploy within this space to help team members reason about the socio-emotional states of other teammates towards the goal of improving perspective-taking and fostering open communication. Our goal in designing the intervention was .....The intervention has three phases. in the first phase each participant reports their own emotions. In the second phase, each participant is asked to reflect on the conversation and guess how each other teammate is feeling. In the final phase, team members receive socio-metric feedback informed by the process \wesley{slightly more details on the socio-metric feedback?}. The self-reports are used to characterize the group climate and each team members' assessments of others' emotions is used in conjunction with their self-reports to provide every team member with a measure of their perceptiveness to others' emotions \wesley{I know what's going on since I did the task but this is still quite a complexed sentence for me to process}. 

To test the efficacy of our intervention, we conduct a controlled-study ($N=110$ in 24 teams) where we compare the benefits of our intervention against the benefits of injecting a reflective pause in team communication. In both conditions, participants recruited from Amazon Mechanical Turk worked synchronously on a decision-making task, in teams of 4-6 via our chat-based collaboration system. Based on the condition assigned to the team, the system injected either the intervention or a reflective pause in the teamwork session. Through surveys at the end of the study, we probed participants for team viability (whether they would consider working with their team gain), perceived conflict, willingness to exchange feedback with team members, and their satisfaction with their team's final solution. 

We find that compared to the control condition, participants in the intervention condition adjudged their teams to be significantly more viable while we found no significant differences in perceived levels of task and relationship conflict. A larger fraction of participants in the intervention condition than the control condition was willing to provide feedback to teammates. Correspondingly a larger fraction of participants in the intervention condition was willing to receive feedback from teammates. Participants in the intervention condition also reported being more significantly more satisfied with their team's final solution than participants in the control condition. Talk about language use differences. \wesley{woohoo great results here, congrats!}

Implications...


Outline options:

% Current:
% 1. Open communication + perspective taking is important but teams don't do it by default because of X and Y
% 2. Other HCI researchers have built systems to improve communication dynamics in teams but they don't solve this problem
% 3. So instead we create this new intervention that attempts to solve the problem
% 4. Solution details
% 5. Results
% 6. Implications- teams convening for the first time etc.

% Guided Deliberation:
% 1. Deliberation is difficult for all teams. Everyone's different opinions can improve outcomes but also lead to conflict. Often people just choose to avoid conflict.
% 2. To derive benefits from the diverse opinions while reducing risks associated with speaking up, we build this intervention


% Remote teams:
% 1. Virtual teams are common
% 2. Open communication + perspective taking is important but teams don't do it by default because of X and Y
% % 2. Seeing people's emotions is hard
% 3. Till now research has focused on providing mechanisms to communicate affect - emojis/GIFs/fonts assuming that people will communicate their emotions and that people can interpret others' emotions
% 4. But the problem is that people don't openly communicate emotions nor is everyone good at reading others. So, we design this intervention to facilitate the process by lowering the barrier to sharing emotions and by making people aware of their inability to read others.

Merged Remote teams:
1. Virtual teams are common
1.5 But systems focus on Task support, but most systems don't care about relational dynamics. 

% Paragraph 2:
2. disagreements + emotions disclosure is important but teams don't do it by default because of X and Y. We call this openness. 
3. Prior work has attempted to address this problem with: 
- The emoji stuff which assumes people will use it spontaneously - which doesn't happen. 
- Proxy work - groupmeter etc. has tried People satisfice and are not critical of others' ideas. 
4. Visualizations and quantification promotes gaming the metrics, and doesn't improve dynamics 

% Paragraph 3:
4. We create a system that allows openness  - disagreements explicit and emotions as well. 
5. Critical insight is creating bounded space - borrowed from Management Science. We make such a space in the online comm channel. 

% Paragraph 4
6. Solution details

7. Results

8. Implications- teams convening for the first time etc. Physical teams?



==> sections-old/01_introductionv2.tex <==
Virtual teams, convened on online platforms, have demonstrated potential to accomplish complex tasks, but are currently limited in their ability to collaborate effectively. Virtual teams have tackled problems ranging from open design~\cite{Salehi2018-vt} to software development~\cite{Valentine2017-qu} and research~\cite{vaish2017crowd}. 
% When tasks can be decomposed into fragments and members' roles can be well defined, virtual teams thrive but when team members need to come together, interact, co-ideate, and deliberate, virtual teams are vulnerable to conflict and misunderstanding. 
However, the reliance on computer-mediated communication makes it difficult to establish communication norms that promote sharing and engaging with each others' ideas and perspectives. 
Computer mediation lowers socioemotional communication and virtual teams tend to be less cohesive than collocated teams, exhibiting lower trust and shared identity~\cite{hinds2003out}. As a result, team members are less likely to speak up and openly express their perspectives~\cite{morrison2011speaking}. 
Furthermore, even when expressed, team members are likely to ignore other team members' perspectives, triggering conflict and threatening the team's performance and sustainability~\cite{hinds2003out}. 

Thus, virtual teams can be even more effective at collaboration if they can use the diverse perspectives and unique expertise of individual members. To do so, team members need to learn to communicate effectively in an open and respectful manner, integrating everyone's perspectives. This problem is even more challenging for teams where team membership often changes, as is common in virtual teams~\cite{Salehi2018-vt, Valentine2017-qu}, For such high-turnover teams, developing effective communication and accommodating new team members is an ongoing challenge. This paper introduces a new system to foster open and ... communication, by creating spaces...

Prior work has attributed the difficulty of establishing healthy communication to the low levels of information richness, lack of social cues, context, and shared emotion in computer-mediated teams~\cite{Hinds2003-ky}. In response to this, researchers have developed new communication channels~\cite{hassib2017heartchat, buschek2015there,lee2006using,wang2004communicating} to increase information richness and novel sociometric feedback mechanisms~\cite{viegas1999chat,tat2002visualising,tat2006crystalchat} to improve social awareness. While these systems enhance awareness about suboptimal behaviors and provide mediums for team members to be more expressive, in practice, several social and psychological barriers prevent team members from using these mechanisms to proactively shape communication norms. Despite the benefits of open and frank communication, team members often do not speak up. When new members are learning to work together in a team, an uncertainty about group norms and potential consequences of speaking up, coupled with lower shared identity, can cause members to view expressing disagreement, voicing concerns, or asking questions as risky. They may believe that their inputs will not be taken seriously~\cite{morrison2011speaking}. All of which discourages team members from speaking up~\cite{morrison2011speaking}. This often leads to unanticipated outcomes: prior work found that when teams were alerted about low group-level agreement as measured in their chat messages, team members responded by passively expressing agreement with each other which led to lower quality work~\cite{Leshed2009-eq}. Such a ``climate of silence''~\cite{Morrison2000-uu} can undermine team performance~\cite{perlow2003silence, argyris1991teaching}.

We leverage the concept of ``spaces''~\cite{zietsma2010institutional, furnari2014interstitial} to foster open and respectful communication by mitigating some of the associated social and psychological barriers. Spaces are social settings separated by physical, temporal or symbolic boundaries from everyday work within which the salience of existing norms and interaction patterns diminishes. This creates an environment conducive to risky and counternormative behaviors that can catalyze the emergence of new dynamics~\cite{Lee2020-zn, bucher2016interplay, furnari2014interstitial, zietsma2010institutional}. This paper introduces a system that leverages spaces in the context of online team communication environments to improve team communication.

 \begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/interfaces.pdf}
    \caption{We introduce a "space" within a chat-based collaboration environment (A) as a temporally and spatially demarcated meta-channel within which team members engage in an intervention aimed at improving perspective-taking and fostering open and respectful communication (B).}
    \label{fig:space}
\end{figure}

We instantiate our "space" as a temporally and spatially demarcated meta-channel within a chat-based collaboration environment (Fig. \ref{fig:space}). We designed and deployed an intervention, within this space, to support processes known to improve perspective-taking while maintaining the ambiguity and anonymity necessary to promote authentic expression. Drawing attention to others' emotions and affective states- \textit{attention modulation}- can increase perspective-taking~\cite{zaki2014empathy,curran2019understanding}. To support this process, we privately elicit how team members actually feel about working with their group and provide the group feedback about the aggregate group climate without revealing individual responses. We also ask each member, in private, to guess how other members might be feeling, to nudge them to direct their attention towards others in the team. Perspective-taking is also regulated by \textit{appraisal} or an individual's evaluation of the authenticity and intensity of others' emotions~\cite{zaki2014empathy}. Emotions expressed privately in the ``space'' are more authentic and uninhibited than those expressed in the chat. So, team members are more likely to recognize potential grievances and act on them when they are confronted with them within the space. Taken together, we expect our intervention to improve perspective-taking and foster open communication. We expect these positive dynamics will also improve team satisfaction and team viability- team members' desire to continue working together.

To test the efficacy of our intervention, we conduct a controlled-study ($N=110$ in 24 teams) where we compare the benefits of our intervention against the benefits of injecting a reflective pause in team communication. In both conditions, participants recruited from Amazon Mechanical Turk worked synchronously on a decision-making task, in teams of 4-6 via our chat-based collaboration system. Based on the condition assigned to the team, the system injected either the intervention or a reflective pause in the teamwork session. Through surveys at the end of the study, we probed participants for team viability (whether they would consider working with their team gain), perceived conflict, willingness to exchange feedback with team members, and their satisfaction with their team's final solution. 

We find that compared to the control condition, participants in the intervention condition adjudged their teams to be significantly more viable while we found no significant differences in perceived levels of task and relationship conflict. Furthermore, we find that participants in the intervention condition were approximately 25.4\% more likely to be willing to provide feedback to teammates than in the control condition (p=0, t(45)=45). Correspondingly a marginally larger fraction of participants in the intervention condition was willing to receive feedback from teammates. Participants in the intervention condition also reported being more significantly more satisfied with their team's final solution than participants in the control condition. Talk about language use differences.

Our findings suggest that embedding computationally-mediated interventions within collaboration environments are a powerful tool in helping teams establish positive interaction norms. Our experiments focused on initial interactions of newly convened remote teams, collaborating over short durations, however, fostering positive interaction dynamics isn't just a one-time process- even long-standing teams are often reconfigured and so, team members have to frequently learn to work with new people. Repeated deployment of the intervention whenever teams experience changes in membership could help teams adapt. While we specifically studied virtual teams, collocated teams also struggle with fostering an environment of open and respectful communication- they could also benefit from computationally-mediated interventions when initially learning to work together.
% When running studies on AMT, the short time frame of the experiment combined with their expectation of future separation causes participants to focus on the completion of the task, while disincentivizing efforts to form cohesive team norms that would only benefit them if they continued working together~\cite{Bradley2003-aa}. Despite this, we were able to observe effects of our intervention 

==> sections-old/01_introductionv3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Yasmine's higher-level notes while reading

%%%% Great work, Pranav!

%%%% I think the introduction could spend a bit more time building up the significance of virtual teams before jumping to the problem statement. For instance, what is it about virtual teams in particular (not just teams in general) that enables this ability to tackle complex tasks?

%%%% After you describe your problem statement ("However, the reliance on..."), your jump to the solution space ("Thus, virtual teams...") reads as fairly disconnected. IOW it is not clear why "diverse perspectives and unique expertise of members" is the hammer you have chosen for your nail. I think this may be remedied by adding adequate depth throughout the beginning of the intro, but I'm happy to take a second pass if you're stuck

%%%% Alright, now that I've read through the paragraphs where you introduce Mindspace ("This paper introduces..." and "Mindspace is motivated..." etc ) I suggest a reworking of the first several paragraphs of the introduction in order to provide adequate depth to motivate this work. See my comments on line 33 and line 39 for additional context/explanation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% it's hard to engage constructively
% 
% 
% 

Virtual teams, convened on online platforms such as/(e.g.,...), have demonstrated the potential to accomplish complex tasks. 

%However,  [??] currently face numerous barriers that prevent them from reaching their fullest collaborative potential. 

For example, virtual teams have tackled problems ranging from open design~\cite{Salehi2018-vt} to software development~\cite{Valentine2017-qu} and research~\cite{vaish2017crowd}. 

%at least one more sentence about the promise of virtual teams, perhaps going into a little more detail about one of the papers you have referenced above 

%here is where I may give one sentence about the unique affordances of computationally-supported teams. In other words, be explicit about what the secret sauce is for why these prior works have been successful. Something like "These benefits are enabled in large part because of distributed nature of team, etc..." but in more refined wording :)

However, the reliance on computer-mediated communication can make it more difficult to establish communication norms that promote sharing and engaging with each others' ideas and perspectives. Computer mediation lowers socioemotional communication [describe what this means]. In addition, virtual teams are less cohesive than collocated teams, exhibiting lower trust and shared identity~\cite{hinds2003out}. As a result, team members are less likely to speak up and openly express their perspectives~\cite{morrison2011speaking}. 
Furthermore, even when team members express their perspectives, these are likely to be ignored by other members, triggering conflict and threatening the team's performance and sustainability~\cite{hinds2003out}.

% There is quite a bit of high-level language used in the following paragraph, and it misses opportunity to provide adequate depth and justification
Thus, virtual teams can be even more effective at collaboration if they can use the diverse perspectives and unique expertise of individual members. To do so, team members need to learn to communicate effectively in an open and respectful manner, integrating everyone's perspectives. Developing these healthy interaction patterns is even more challenging for teams where membership often changes, as is common in virtual teams~\cite{Salehi2018-vt, Valentine2017-qu}, For such high-turnover teams, developing effective communication and accommodating new team members is an ongoing challenge. 

This paper introduces \sys{}, a chat-embedded intervention designed to help virtual teams engage in processes known to improve perspective-taking while still maintaining the ambiguity and anonymity necessary to promote authentic expression. Such authentic perspective-taking, in turn, improves work satisfaction and encourages more open communication and feedback within the team.
% This paper introduces a new system to foster open and ... communication, by creating spaces...

% Aha! The following two paragraphs include well-written motivations of your problem statement and the solution space. To be honest, I think my concerns above can be addressed in large part by reworking the introduction to include these details earlier.
\sys{} is motivated by prior work that has attributed the difficulty of establishing healthy communication in virtual teams to both technical and organizational challenges. From a technical perspective,  the low levels of information richness, lack of social cues, context, and shared emotion in computer-mediated teams hinder communication~\cite{Hinds2003-ky}. However, social and psychological barriers among team members make it challenging to improve the levels of information richness and context. For instance, teams in practice have been reluctant to adopt new communication channels  that communicate nuanced social cues such  as bio-signals~\cite{hassib2017heartchat, wang2004communicating}   kinetic typography~\cite{buschek2015there,lee2006using}, or even novel sociometric feedback mechanisms~\cite{viegas1999chat,tat2002visualising,tat2006crystalchat}. 
% can improve social awareness. In practice, however,  social and psychological barriers prevent team members from using these mechanisms to proactively shape communication norms. 

From an organizational perspective, prior work notes that even when team members are immersed in an information-rich social context, a ``climate of silence''~\cite{Morrison2000-uu} can undermine team performance~\cite{perlow2003silence, argyris1991teaching}. When new members are learning to work together in a team, an uncertainty about group norms and potential consequences of speaking up, coupled with lower shared identity, can cause members to view expressing disagreement, voicing concerns, or asking questions as risky. They may believe that their inputs will not be taken seriously~\cite{morrison2011speaking}. All of which discourages team members from speaking up~\cite{morrison2011speaking}. This often leads to unanticipated outcomes: prior work found that when teams were alerted about low group-level agreement as measured in their chat messages, team members responded by passively expressing agreement with each other which led to lower quality work~\cite{Leshed2009-eq}. 

% If you decide to rework the introduction as suggested above, I believe you could introduce your system in this paragraph, rephrasing slightly what you have below.
In response, \sys{} leverages the construct of ``spaces''~\cite{zietsma2010institutional, furnari2014interstitial} from organizational science research. Spaces foster open and respectful communication by mitigating some of the associated social and psychological barriers. Spaces are social settings separated by physical, temporal or symbolic boundaries from everyday work within which the salience of existing norms and interaction patterns diminishes. This creates an environment conducive to risky and counternormative behaviors that can catalyze the emergence of new dynamics~\cite{Lee2020-zn, bucher2016interplay, furnari2014interstitial, zietsma2010institutional}. While spaces have been mostly studied among co-located teams, \sys{} leverages spaces in the context of online team communication environments to improve team communication.

 \begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/interfaces.pdf}
    \caption{(A) Virtual teams often co-ordinate and communicate over chat. \sys{} helps teams establish positive interaction norms that promote sharing and engaging with each others perspectives. (B) When triggered, \sys{ } appears as a widget in the chat interface and disables the chat while teams carry out a perspective-taking exercise. The perspective-taking exercise in \sys{} attempts to make team members more attuned to each others' emotions by prompting them to reflect on how others' might be feeling and by providing them with socio-metric feedback on group climate and their perceptiveness to their teammates emotions. We find that \sys{} improves work satisfaction and encourages more open communication and feedback within the team}
    \label{fig:space}
\end{figure}

\sys{} instantiates a norm-diminished "space" through temporally and spatially separated channel within a chat-based collaboration environment (Fig. \ref{fig:space}). We designed and deployed the norm-diminished spaces within \sys{} to support processes known to improve perspective-taking while maintaining the ambiguity and anonymity necessary to promote authentic expression. 

% Drawing attention to others' emotions and affective states- \textit{attention modulation}- can increase perspective-taking~\cite{zaki2014empathy,curran2019understanding}. 

% To support this process, we privately elicit how team members actually feel about working with their group and provide the group feedback about the aggregate group climate without revealing individual responses. We also ask each member, in private, to guess how other members might be feeling, to nudge them to direct their attention towards others in the team. Perspective-taking is also regulated by \textit{appraisal} or an individual's evaluation of the authenticity and intensity of others' emotions~\cite{zaki2014empathy}. Emotions expressed privately in the ``space'' are more authentic and uninhibited than those expressed in the chat. So, team members are more likely to recognize potential grievances and act on them when they are confronted with them within the space. Taken together, we expect our intervention to improve perspective-taking and foster open communication. We expect these positive dynamics will also improve team satisfaction and team viability- team members' desire to continue working together.

To test the efficacy of our intervention, we conducted a controlled-study ($N=110$ in 24 teams) where we compared the benefits of our intervention against the benefits of injecting a reflective pause in team communication. In both conditions, participants recruited from Amazon Mechanical Turk worked synchronously on a decision-making task, in teams of 4-6 via our chat-based collaboration system. 
% Participants were randomly assigned to a control condition that injected a reflective pause in the teamwork session, or a \sys{} condition that injected the ``spaces" channel. Through surveys at the end of the study, we probed participants for team viability (whether they would consider working with their team gain), perceived conflict, willingness to exchange feedback with team members, and their satisfaction with their team's final solution. 

We found that compared to a control condition, participants in the \sys{} condition were significantly more satisfied with their team's solution and they judged their teams to be significantly more viable. Furthermore, we find that participants in the \sys{} condition were approximately 25.4\% more likely to be willing to provide feedback to teammates than in the control condition, and a larger fraction of participants  were willing to receive feedback from teammates. At the same time, we found no significant differences in perceived levels of task and relationship conflict, suggesting that the open communication facilitated by \sys{} did not translate to greater conflict. Analyzing LIWC indicators for teams in the two conditions, we find that \sys{} increased teams' usage of second-person pronouns suggesting that the conversation was more other-focused. \sys{} also led to an increase in informality and netspeak in the teams' chatlogs suggesting that teammembers formed stronger social bonds.  

Our findings suggest that embedding computationally-mediated interventions within collaboration environments are a powerful tool in helping teams establish positive interaction norms. Our experiments focused on initial interactions of newly convened remote teams, collaborating over short durations. However, fostering positive interaction dynamics isn't just a one-time process- even long-standing teams are often reconfigured and so, team members have to frequently learn to work with new people. Repeated deployment of the intervention whenever teams experience changes in membership could help teams adapt. While we specifically studied virtual teams, collocated teams also struggle with fostering an environment of open and respectful communication- they could also benefit from computationally-mediated interventions when initially learning to work together.

==> sections-old/01_introductionv4.tex <==
Despite their inherent promise, virtual teams \pranav{stronger grounding for what these virtual teams are}, convened on online platforms have had limited success. Researchers suggest that such Flash Teams~\cite{Retelny2014-gk} and Flash Organizations~\cite{Valentine2017-qu}, through their ``computationally-represented structures'' will result in a world where ``anyone with an internet connection can assemble an organization from an online labor market and then lead that organization in pursuit of complex, open-ended goals''~\cite{Valentine2017-qu}.  Unfortunately, the evidence so far is decidedly mixed. Virtual teams have indeed tackled problems ranging from software development~\cite{Valentine2017-qu} to research~\cite{vaish2017crowd},  but only when these goals can themselves be decomposed into tasks that \textit{individual} workers can accomplish. When virtual teams engage in tasks that cannot be decomposed, where team members need to \textit{collectively} ideate, engage with each others' perspectives, and make decisions, they often fail: either through poor performance~\cite{bjelland2008inside}, inter-team conflict conflict~\cite{kittur2007he}, and in the extreme, because team members refuse to work with each other again~\cite{Whiting2019-wl}.

A possible response to these disappointing findings is to design systems that make disagreements and conflicts between team members less frequent, so teams are more likely to succeed. Unfortunately, disagreements are often the result of diverse perspectives and ideas of individual members~\cite{Sessa1996-ba}, and so eliminating disagreements may well eliminate these diverse contributions as well. Prior work shows the disagreement is in fact a double-edged sword: when managed well, open communication of disagreement and alternate ideas can improve collaboration~\cite{Menold2019-wc, Morrison2000-uu}. When managed poorly, disagreement can spiral out of control, triggering interpersonal conflict~\cite{kittur2007he, Whiting2019-wl}. 

Thus, when teams need to accomplish tasks that benefit from the diverse perspectives of members, require negotiation, and collective decision-making, surfacing and managing team friction is crucial. Specifically,  members need to be able to communicate opinions openly but without such conflicts of opinion impairing teams. While all teams struggle to strike this balance, but lack of richness of computer-mediated communication compared to face-to-face communication exacerbates this problem for virtual teams. Without such balance, virtual teams are prone either to social loafing where team members avoid speaking up and voicing their opinions~\cite{kim2021moderator}, or where team members  ignore other members'  their perspectives, triggering conflict and threatening the team's performance and sustainability~\cite{hinds2003out}.


 \begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/interfaces.pdf}
    \caption{(A) Virtual teams often co-ordinate and communicate over chat. \sys{} helps teams establish positive interaction norms that promote sharing and engaging with each other's perspectives. (B) When triggered, \sys{ } appears as a widget in the chat interface and disables the chat while teams carry out a perspective-taking exercise. The perspective-taking exercise in \sys{} attempts to make team members more attuned to each others' emotions by prompting them to reflect on how others' might be feeling and by providing them with socio-metric feedback on group climate and their perceptiveness to their teammates emotions. We find that \sys{} improves work satisfaction and encourages more open communication and feedback within the team}
    \label{fig:space}
\end{figure}


To help members of virtual teams engage constructively with each others' perspectives, this paper introduces \sys{}, a chat-embedded intervention that attempts to mitigate some of the social and psychological barriers to open team communication. Specifically, \sys{} identifies two potential barriers based on literature in organizational psychology. The first barrier is that groups require a climate of \textit{safety} and \textit{efficacy} for members to speak up- team members speak up only when they feel their opinion matters (\textit{efficacy}) , that it is safe to voice their opinion (\textit{safety}), and that their opinions will be taken into account (\textit{efficacy})~\cite{morrison2011speaking}. The second barrier is that that team norms can be hard to reset mid-interaction~\cite{marks2001temporally, Whiting2020-pq}. In response, \sys{} induces perspective-taking as a useful tool to maintain the \textit{safety} and \textit{efficacy} essential for team members to engage with each other. To overcome the inertia of norms, transform established norms and cultivate \textit{safety} and \textit{efficacy} by inducing perspective-taking, \sys{} leverages the power of ``experimental spaces''~\cite{zietsma2010institutional, furnari2014interstitial}. Spaces are social settings separated by physical, temporal or symbolic boundaries from everyday work within which the salience of existing norms and interaction patterns diminishes. This creates an environment conducive to risky and counternormative behaviors that can catalyze the emergence of new dynamics~\cite{Lee2020-zn, bucher2016interplay, furnari2014interstitial, zietsma2010institutional}. While spaces have been mostly studied among co-located teams, \sys{} leverages spaces in the context of online team communication environments to induce perspective-taking and transform team communication. This in turn, improves work satisfaction and encourages more open communication and feedback within the team, and boosts teams' desire to continue working together-\, i.e. team viability.

\sys{} instantiates a norm-diminished "space" through temporally and spatially separated channel within a chat-based collaboration environment (Fig. \ref{fig:space}). Within \sys{}, we orchestrate an exercise aimed at inducing perspective-taking. 

In doing so, \sys{} shifts the focus from easily observable team communication patterns to the subtle (but vitally important) social and psychological barriers preventing team members from changing these patterns. For instance, prior work has highlighted problematic communication patterns by providing sociometric feedback~\cite{Leshed2007-up,Kim2012-jv,Leshed2009-eq,Tausczik2013-br} and by making explicit recommendations for behavior change ~\cite{Tausczik2013-br, kim2021moderator}. In short, these systems assume that highlighting problematic patterns and suggesting changes is sufficient to transform behaviors. However, because they ignore the social and psychological barriers preventing team members from speaking up, they often have adverse outcomes: a system that displayed group-level agreement led to team members expressing agreement with a majority opinion even if they did not agree with it, in attempts to improve displayed agreement~\cite{Leshed2009-eq}. 
% With \sys{}, we suggest that focusing on the barriers to changing communication patterns is a more effective lever for technological support, as it provides scaffolding for behavior change, but still allows teams to self-regulate their communication. 

To test the efficacy of our \sys{}, we conducted a controlled-study ($N=110$ in 24 teams) where we compared the benefits of \sys{} against an alternative intervention in which participants simply reflected on their team experience. In both conditions, participants recruited from Amazon Mechanical Turk worked synchronously on a decision-making task, in teams of 4-6 via a chat-based collaboration system. 

We found that participants in the \sys{} condition were significantly more satisfied with their team's solution and they judged their teams to be significantly more viable. Furthermore, we find that participants in the \sys{} condition were approximately 25.4\% more likely to be willing to provide feedback to teammates than in the control condition, and a larger fraction of participants  were willing to receive feedback from teammates. At the same time, we found no significant differences in perceived levels of conflict, suggesting that the open communication facilitated by \sys{} did not translate to greater conflict. Analyzing linguistic patterns exhibited  by teams during deliberation in the two conditions, we find that \sys{} increased teams' usage of second-person pronouns, suggesting that the conversation was more other-focused. \sys{} also led to an increase in informality and netspeak in the teams' chatlogs suggesting that team members formed stronger social bonds.

Our findings suggest that embedding computationally-mediated interventions within collaboration environments is a powerful tool in helping teams establish positive interaction norms. Our experiments focused on initial interactions of newly convened remote teams, collaborating over short durations. However, fostering positive interaction dynamics isn't just a one-time process- even long-standing teams are often reconfigured and so, team members have to frequently learn to work with new people. Repeated deployment of the intervention whenever teams experience changes in membership could help teams adapt. While we specifically studied virtual teams, collocated teams also struggle with fostering an environment of open and respectful communication- they could also benefit from computationally-mediated interventions when initially learning to work together.

==> sections-old/02_related.tex <==
This research contributes to a growing body of work that aims to improve collaboration experiences of computer-mediated teams, tying together research in organizational behavior with research in HCI. We start by reviewing existing HCI research on software support for teams and highlight the need for systems that foster positive interaction norms. Drawing on research in organizational behavior, we attempt to characterize interaction patterns of performant and sustainable teams. We then look at how we can design effective interventions to cultivate these constructive interaction patterns in teams.     

\subsection{Beyond team assembly and task support: designing systems to nurture teams}
To improve outcomes of computer-mediated teams, human-computer interaction researchers have developed several systems aimed at assembling the right team for the task. Prior work has shown that teams composed of members with higher skill diversity~\cite{horwitz2007effects}, demographic diversity~\cite{lykourentzou2016personality}, and differing personality types~\cite{bear2011role} perform better and are more satisfied. Consequently, researchers have developed systems that optimize for these criteria and assemble teams with the most promise for success. Researchers have also built team-dating systems to improve collaboration by allowing people to experience work with different collaborators before team formation~\cite{Lykourentzou2017-yz}. Simultaneously, rotating members strategically can promote mixing of ideas~\cite{Salehi2018-vt}. To allow teams to cope with evolving work, researchers have also designed systems to on-board experts on-demand~\cite{Valentine2017-qu, Retelny2014-gk}. However, while these systems have demonstrated success in identifying good collaborators, team composition is naturally constrained by availability of talent. How can we help \textit{any} team achieve their full potential and work effectively?

One way to help computer-mediated teams work effectively is to provide support for task completion and coordination of effort. HCI researchers have designed several systems to support team tasks. This includes systems to create and manage workflows~\cite{Valentine2017-qu, rahman2020mixtape}, systems to structure interaction between collaborators~\cite{park2021facilitating, rahman2020mixtape}. These systems decompose work into tasks that can be handled individually by members. As such, they reduce the amount of task planning that teams need to do and lower the need for members to communicate with each other. Consequently, when tasks can be decomposed into independent fragments and members' roles can be well defined, these systems allow virtual teams thrive. When tasks can not be completely compartmentalized and members need to come together, interact, co-ideate, and deliberate, computer-mediated teams are once again vulnerable to conflict and misunderstanding~\cite{Whiting2019-wl, Whiting2020-pq}.

Healthy team communication is key to ensuring team viability. One prior study found that while task-support interventions improved the performance of participant teams on average, interpersonal conflict in some teams negated the positive effects of the intervention~\cite{Bradley2003-aa}. Teams with healthy interpersonal processes provide a fertile ground for the positive impact of task-support interventions to improve performance further. Without effective communication, team performance can suffer and can even lead to teams not wanting to continue working together. Furthermore, team performance alone doesn't paint a complete picture of how a collaboration is going. Even high performing teams might have might have toxic culture, unresolved conflict, divisive interactions, and member burnout. For a more holistic evaluation of a team, it is important to look beyond just \textit{team performance} and evaluate \textit{team viability}: the team's sustainability and capacity for continued success~\cite{Bell2011-rz,Cooperstein2017-cj, Whiting2019-wl}. Team viability is an emergent state that captures the potential of the team to continue performing well, the desire of the team to continue working together, and the extent to which the team can adapt to changing circumstances~\cite{Bell2011-rz}. Antecedents of team viability include perceived performance and interpersonal friction~\cite{Cooperstein2017-cj}. Consequently, viability requires that in addition to being performant, teams also have healthy communication and interpersonal processes in place~\cite{Cooperstein2017-cj}.

\subsection{The right amount of team-friction: identifying interaction patterns of viable teams}
% Interventions focused on improving interaction patterns in teams typically aim to improve positive exchanges in teams characterized by positive emotion and agreement~\cite{Tausczik2013-br}. However, research on what constitutes constructive team-communication patterns suggests that teams need to have the right amount of friction.
Research on what constitutes constructive team-communication patterns suggests that teams need to have the right amount of friction. Too much disagreement, unresolved conflict and disregard for others' opinions and criticism can trigger negative emotions, causing members to get angry and distressed~\cite{Jung2015-px}. This can spiral out of control~\cite{Jung2015-px} and lead to a loss of viability. Too little disagreement and critical communication is also bad and can impair team performance~\cite{perlow2003silence, argyris1991teaching}, team satisfaction and consequently, viability. Eliciting diverse perspectives by fostering open communication of ideas, opinions, and issues, can help uncover new solutions~\cite{Menold2019-wc}, improve decision making, facilitate team learning~\cite{morrison2011speaking, Morrison2000-uu}, and help identify problems. However, for teams to cultivate, and benefit from, this right amount of friction- where members communicate opinions openly but opinion conflicts don't hinder teams- they need ensure that members feel it is both \textit{safe} and \textit{effective} to voice their opinions~\cite{morrison2011speaking}. 

Team members feel \textit{safe} expressing themselves when they do not anticipate potential negative consequences of speaking up~\cite{morrison2011speaking}- they shouldn't be attacked or chastised for speaking up. However merely cultivating the safety necessary for people to express opinions is not enough; to improve outcomes, team members must also engage with others' perspectives, foster inclusivity, and affirm each other~\cite{Salehi2018-vt, Carmeli2015-qv, Hoever2012-hn}. This not only allows teams to incorporate diverse opinions of members but also signals to members that their opinions will be taken into account and acted upon. This can convince members that voicing their opinions is an \textit{effective} way to enact change and in turn motivates them continue to voice their opinions. The diverse perspectives and unique expertise of individual members make teams potent and so, for teams to be effective it is crucial that team-members both speak up, expressing their perspectives, and that they listen to and engage with others' perspectives, in a respectful manner~\cite{morrison2011speaking}.

% A large body of work in organizational behavior has shown that positive relational dynamics are crucial for healthy functioning of teams~\cite{Lee2020-zn}. Respect, openness, connectedness, effective conflict management, and affect management can improve team creativity~\cite{Carmeli2015-qv}, resilience~\cite{Stephens2013-vx}, performance~\cite{Carmeli2015-qv,Edmondson1999-wl}, and ultimately, viability. Respectful interactions including engaging with the diverse perspectives of team members, ensuring inclusivity, and making sure people’s ideas and opinions are respected~\cite{Lee2020-zn} lead to higher cohesion and creativity~\cite{Carmeli2015-qv}. Teams with higher psychological safety and open communication place value on critical communication. Such open communication of disagreement and issues can lead to enhanced performance~\cite{Edmondson1999-wl} and decision making~\cite{Morrison2000-uu}. 

HCI researchers have developed methods to detect whether the interaction patterns in a team are healthy~\cite{Vrzakova2019-vk,Stewart2019-cs}. They have developed models that can leverage information about facial expression, eye gaze, head movements, speech, text, physiology, and interaction to detect the presence of positive traits~\cite{Cao2021-gm,Stewart2019-cs,Vrzakova2019-vk} such as turn-taking~\cite{Jokinen2013-ai}, interactivity~\cite{Ashenfelter2007-tk}, high-levels of empathy~\cite{Ishii2018-ex}, and team cohesion~\cite{Muller2018-ed}. These models have also enabled predicting team performance and team viability from a team’s interactions~\cite{Cao2021-gm}. While this line of work has furthered our understanding of which interpersonal processes and behaviors promote team viability, cultivating these prosocial behaviors in teams remains challenging~\cite{Lee2020-zn}. Our work attempts to move from these descriptive insights towards prescriptive interventions to help teams develop positive communication patterns.  

\subsection{Fostering constructive interaction patterns in teams}
Prior work has attributed the difficulty of establishing healthy communication to the low levels of information richness, lack of social cues, context, and shared emotion in computer-mediated teams~\cite{Hinds2003-ky}. In response, researchers have developed more information rich communication channels to improve social cues and emotional expression in these messaging systems. This includes systems to communicate affect by altering the font and animation of text~\cite{buschek2015there,lee2006using,wang2004communicating}, and via abstract visuals~\cite{viegas1999chat,tat2002visualising,tat2006crystalchat}. Researchers have also explored the design of computer-mediated interventions to nudge people towards more positive interaction patterns by providing them socio-metric feedback on group communication patterns~\cite{Leshed2007-up,Kim2012-jv,Leshed2009-eq,Tausczik2013-br}. Some tools go beyond making extant behaviors salient and also make specific recommendations on how teams should alter their practices to move them closer to desired behaviors~\cite{Tausczik2013-br, kim2021moderator}. However, these systems have only had limited success, because they assume that highlighting problematic patterns and providing information-rich communication channels is sufficient to nudge team members to express their authentic opinions and change their interaction norms. In doing so, they ignore the social and psychological barriers preventing team members from speaking up: they do nothing to alter team members' perceived \textit{safety} and \textit{efficacy} of speaking up, necessary for open and healthy team communication. This can lead to undesirable outcomes: prior work found that visualizing group-level agreement led to a form of social loafing where team members expressed agreement with the majority opinion even if they did not agree with it with it and this ultimately resulted in lower quality work~\cite{Leshed2009-eq}.

Transforming and shaping interaction norms to promote open and respectful communication is challenging. It requires team members to take initiative and proactively engage in open and frank communication but team members often do not speak up. They may view expressing disagreement, voicing concerns, or asking questions as risky (low levels of perceived \textit{safety}) or they may believe that their inputs will not be taken seriously~\cite{morrison2011speaking} (low levels of perceived \textit{efficacy}) pushing them to avoid disagreeing entirely. These beliefs about speaking up are shaped by the interaction history of the team~\cite{morrison2011speaking}. For newly convened teams, an uncertainty about group norms and potential consequences of speaking up could lead to low perceived \textit{safety} and discourage employees from speaking up. Team members who do not strongly identify with their team, or who are unsatisfied with their team, might perceive low levels of \textit{efficacy} and think speaking up is futile~\cite{morrison2011speaking}. In such cases, a ``climate of silence''~\cite{Morrison2000-uu} becomes the norm which can undermine team performance and viability~\cite{perlow2003silence, argyris1991teaching}. 

\subsection{Psychological theories informing the design of our intervention}
To design an intervention to promote more constructive communication behaviors, we draw on perspective-taking as a useful tool to \textit{maintain} the \textit{safety} and \textit{efficacy} needed for healthy team communication. To support the \textit{development} of perspective-taking and positive team dynamics, we create an environment that is conducive to the emergence of new practices. We do this by creating a new ``space'' that provides a zone of \textit{safety} for experimental behaviors where teams can engage in a perspective-taking exercise.

\subsubsection{Inducing perspective-taking to maintain \textit{safety} and \textit{efficacy}}

Perspective-taking can be a useful tool to maintain perceived \textit{safety} of speaking up. By taking another’s perspective, team members are more likely to anticipate disagreement, recognizing that other people will have different views~\cite{Sessa1996-ba}. This can both reduce initial opposition to someone else's ideas as well as mentally prepare individuals to handle opposition to their ideas. Both of these together contribute to \textit{safety}.

Perspective-taking encompasses considering others’ evaluative standards which can lead to better evaluation of their ideas and more constructive feedback~\cite{Hoever2012-hn}. This can help team members feel heard and contribute to improved perceptions of \textit{efficacy}. Trying to understand someone else’s perspective can also trigger clarifying communication that can ultimately facilitate better understanding of everyone’s ideas~\cite{Hoever2012-hn}. Perspective-taking can lead to a cognitive reframing that leads to better integration of others’ ideas~\cite{Hargadon2006-ri}. Taken together, this suggests that perspective-taking can help teams take everyone's opinions into account and make everyone feel heard, both of which improve perceived \textit{efficacy} of speaking up.

\subsubsection{Creating an experimental space to induce perspective-taking} To suspend pre-existing interaction norms and induce perspective-taking, we draw on work that has explored the benefits of creating “spaces'' for transformative dialogue~\cite{Lee2020-zn, zietsma2010institutional}. Spaces are social settings separated by physical, temporal or symbolic boundaries from everyday work within which the salience of existing norms and interaction patterns diminishes. This creates an environment conducive to risky and counternormative behaviors that can catalyze the emergence of new dynamics~\cite{Lee2020-zn, bucher2016interplay, furnari2014interstitial, zietsma2010institutional}. Examples of such spaces include creating meetings to specifically engage in discussion about work challenges or organizing a retreat to help team members connect outside of work environments. Such “experimental spaces'' have been effective at reducing barriers to open communication in teams and consequently, fostering positive relational dynamics~\cite{Lee2020-zn}. We attempt to imagine what such a space might look like in the context of online team communication environments and how we might use such a space to induce perspective-taking towards the goal of improving team interactions.



==> sections-old/02_relatedv1.tex <==
\subsection{Healthy interpersonal processes in teams}
A large body of work in organizational behavior has shown that positive relational dynamics are crucial for healthy functioning of teams~\cite{Lee2020-zn}. Respect, openness, connectedness, effective conflict management, and affect management can improve team creativity~\cite{Carmeli2015-qv}, resilience~\cite{Stephens2013-vx}, performance~\cite{Carmeli2015-qv,Edmondson1999-wl}, and ultimately, viability. Respectful interactions including engaging with the diverse perspectives of team members, ensuring inclusivity, and making sure people’s ideas and opinions are respected~\cite{Lee2020-zn} lead to higher cohesion and creativity~\cite{Carmeli2015-qv}. Teams with higher psychological safety and open communication place value on critical communication. Such open communication of disagreement and issues can lead to enhanced performance~\cite{Edmondson1999-wl} and decision making~\cite{Morrison2000-uu}. 

Armed with this understanding, CSCW researchers have developed methods to detect the presence or absence of these healthy interpersonal processes in communication traces generated by teams~\cite{Vrzakova2019-vk,Stewart2019-cs}. Rooted in an understanding of the underlying socio-cognitive processes, researchers have developed models that can leverage information about facial expression, eye gaze, head movements, speech, text, physiology, and interaction to detect the presence of positive traits~\cite{Cao2021-gm,Stewart2019-cs,Vrzakova2019-vk} such as turn-taking~\cite{Jokinen2013-ai}, interactivity~\cite{Ashenfelter2007-tk}, high-levels of empathy~\cite{Ishii2018-ex}, and team cohesion~\cite{Muller2018-ed}. These models have also enabled predicting team performance and team viability from a team’s interactions~\cite{Cao2021-gm}. While this line of work has furthered our understanding of the interpersonal processes and behaviors that are promotive of group efficacy, there is very little work that examines how we might actually cultivate these prosocial behaviors in teams~\cite{Lee2020-zn}. How do we translate these descriptive insights into prescriptive interventions? While we can use these insights to assemble effective teams by evaluating mutual compatibility of members, how can we help teams that have already been convened, develop positive interpersonal processes? How can we help teams break out of maladaptive interaction patterns and nudge them towards positive interaction patterns? 

\subsection{Interventions to improve interpersonal processes in teams}
To catalyze the cultivation of positive relational dynamics, researchers have explored the design of behavioral protocols- interventions- that improve interpersonal processes in teams and help teams overcome negative interaction patterns that might have been established previously~\cite{Lee2020-zn,Leshed2007-up,Whiting2020-pq}. Interventions in the organizational behavior literature typically take the form of training sessions that aim to improve the soft skills of team members~\cite{Hoever2012-hn,Sessa1996-ba}. More recently, researchers have explored the benefits of creating “spaces'' for transformative dialogue and interaction scripts to govern behaviors of people within these “spaces''~\cite{Lee2020-zn}. Examples of such spaces include creating meetings to specifically engage in discussion about work challenges or organizing a retreat to help team members connect outside of work environments. Such “experimental spaces'' and scripts have been effective at reducing barriers to open communication in teams and consequently, fostering positive relational dynamics~\cite{Lee2020-zn}.  

As computer-mediated collaboration has become increasingly dominant and teams often collaborate remotely, researchers have developed computer-mediated interventions to support teamwork. Some of these interventions and tools focus on providing feedback on teamwork practices as a mechanism to improve collaborative skills~\cite{He2017-xw,Leshed2007-up}. Researchers have built tools that automatically detect and provide sociometric feedback on group communication patterns~\cite{Kim2012-jv,Leshed2009-eq,Tausczik2013-br}. This can help teams identify suboptimal group dynamics and move towards more positive communication patterns. In addition to automated feedback, prompting team members to reflect on that feedback can also improve levels of empathy in teams~\cite{He2017-xw}. 

Some interventions move beyond making extant behaviors salient and also make specific recommendations on how teams should alter their practices to move them closer to desired behaviors~\cite{Tausczik2013-br,Zhou2018-mk}. Visualizing peer feedback on teamwork practices is also effective at promoting more cooperative behaviors~\cite{Leshed2007-up}. Recognizing that early interaction can derail teams, researchers have also explored repeatedly reconvening the same team in its initial phases to prevent it from getting stuck with maladaptive interaction patterns~\cite{Whiting2020-pq}. Complementing this body of work, we focus on a mechanism that is fundamental to effective teamwork--- perspective taking.

\subsection{Harnessing diverse perspectives of team members}
Teams are potent largely because of the diverse perspectives and ideas of individual members. These diverse perspectives and opinions often trigger disagreement or conflict on problem solving tasks. Such conflict is inherent to problem solving~\cite{Paletz2017-fh} and when harnessed can improve creative outcomes of groups and is ultimately what makes teams effective~\cite{Paletz2017-fh,Salehi2018-vt,Sessa1996-ba}. Diversity in perspectives can enhance creative outcomes as minority perspectives can lead to exploration of alternate solutions~\cite{Menold2019-wc, Sauer2006-rp} Thus, cognitive diversity is considered an asset when assembling teams. If not managed effectively, however, conflict can trigger negative emotions causing members to get angry and distressed~\cite{Jung2015-px}. Negative emotions also have a tendency to escalate and spiral out of control~\cite{Jung2015-px}. Such interpersonal friction can impair performance and threaten team viability~\cite{Cooperstein2017-cj}. Computer-mediated teams are especially vulnerable: they are rife with misunderstanding~\cite{Hinds2003-ky}. To be successful, it is important for teams to integrate perspectives of all team members and to navigate the resulting conflict effectively~\cite{Hoever2012-hn}. Perspective-taking is a tool that can help teams on both fronts. 

Diverse perspectives do not automatically result in improved creativity~\cite{Dahlin2005-kc}. To capitalize on the diversity, team members need to invest cognitive energy to understand their teammates’ approaches to the task~\cite{Hoever2012-hn}. The other-focused nature of perspective-taking makes it a valuable tool for facilitating comprehensive evaluation of others’ ideas. Perspective-taking also encompasses considering others’ evaluative standards which can lead to better evaluation of their ideas and more constructive feedback. Trying to understand someone else’s perspective can also trigger clarifying communication that can ultimately facilitate better understanding of everyone’s ideas~\cite{Hoever2012-hn}. Finally, perspective-taking can lead to a cognitive reframing that leads to better integration of others’ ideas~\cite{Hargadon2006-ri}.

Perspective-taking can also help teams deal with conflict effectively~\cite{Sessa1996-ba}. Conflict is typically characterized as either task-conflict or relationship-conflict~\cite{Jung2015-px,Sessa1996-ba}. Task conflict refers to disagreement between team members about ideas or processes concerning the task the team is working on~\cite{Sessa1996-ba,Jung2015-px}. Relationship conflict is people-oriented as opposed to task-oriented and includes questioning competence of others, struggling for leadership, unbalanced contributions, and personal incompatibilities~\cite{Sessa1996-ba}. While task-conflict - inherent to collaborative problem solving- can lead to improved outcomes and is associated with triggering positive affect, relationship conflict can lead to negative affect and threaten team viability~\cite{Sessa1996-ba}. However, these differences in conflict are far from salient: team communication is fallible and often leads to misunderstandings~\cite{Hinds2003-ky,Jung2015-px}. Team members might mistakenly perceive the conflict to be directed towards them instead of the task~\cite{Sessa1996-ba}. Perspective-taking can mitigate some of these problems. By taking another’s perspective, team members are more likely to anticipate disagreement, recognizing that other people will have different views. By trying to understand how others think and feel about the situation and why they are behaving a certain way, team members will find it easier to discern the source of the conflict. This can lead to decreased perceptions of relationship conflict in the group and can help teams effectively navigate conflict~\cite{Sessa1996-ba}. 

\subsection{Embedding perspective-taking interventions within collaboration environments}
Contrary to classical assumptions, a person's ability to take-perspectives is not an immutable trait~\cite{zaki2014empathy,curran2019understanding} and can be regulated by \textit{attention modulation}: drawing attention to others' emotions and affective states can increase perspective-taking~\cite{zaki2014empathy,curran2019understanding}. Perspective-taking is also regulated by \textit{appraisal} or an individual's evaluation of the authenticity and intensity of others' emotions~\cite{zaki2014empathy}. People might often choose to misrepresent their true emotions to adhere to social display rules and so, cues taken at face value might not accurately represent the target's true affective states~\cite{ansfield2007smiling,ekman1997smiles}. Enabling people to accurately appraise affective meaning of others' cues can improve perspective-taking. Taken together, this suggests the need for 1) communication channels that make people more attuned to others' affective states, 2) aids to augment people's ability to accurately assess others' affective states, and 3) interventions that lower the social and psychological barriers preventing people from expressing their true affective states.

Instant messaging environments such as Slack, Skype, Teams, and Hangouts that house team communication and collaboration and several researchers have explored ways to improve emotional awareness and expressiveness in these messaging systems~\cite{hassib2017heartchat}. This includes systems that communicate affect and context by altering the font and animation of text~\cite{buschek2015there,lee2006using,wang2004communicating}, via abstract visuals~\cite{viegas1999chat,tat2002visualising,tat2006crystalchat} and more recently, by  

These systems make 2 key assumptions- that people will express their true emotions and that true emotions can be inferred from text.




==> sections-old/02_relatedv2.tex <==
This research contributes to a growing body of work that aims to improve collaboration experiences of computer-mediated teams, tying together research in organizational behavior with research in HCI. We contextualize our work by reviewing existing HCI research on software support for teams and understanding unsupported team-development processes. We review research on identifying healthy team-interaction patterns to understand factors that contribute to constructive team communication. To understand available mechanisms to shape teams' interactions, we look at existing work on fostering healthy team practices. Finally, we motivate the design of our intervention by illustrating the role of experimental spaces in enabling counternormative behaviors and perspective-taking in promoting prosocial team behaviors and enhancing collaboration experiences.

\subsection{Beyond team assembly and task support- designing systems to nurture teams}
To improve outcomes of computer-mediated teams, human-computer interaction researchers have developed several systems aimed at assembling the right team for the task and providing teams with software support to succeed at the given task. Systems for team assembly aim to identify teams that show the most promise for success. Teams composed of members with higher skill diversity~\cite{horwitz2007effects}, demographic diversity~\cite{lykourentzou2016personality}, and differing personality types~\cite{bear2011role} perform better and are more satisfied. Allowing people to experience work with different collaborators before team formation can improve collaboration~\cite{Lykourentzou2017-yz}. Simultaneously, rotating members strategically can promote mixing of ideas~\cite{Salehi2018-vt}. To allow teams to cope with evolving work, researchers have also designed systems to on-board experts on-demand~\cite{Valentine2017-qu, Retelny2014-gk}. However, while these systems have demonstrated success in identifying good collaborators, team composition is naturally constrained by availability of talent. How can we help \textit{any} team achieve their full potential and work effectively?

Team assembly is just the initiation of collaboration and so, to support teams once convened, HCI researchers have designed several systems to support team tasks. This includes systems to create and manage workflows [Flash, mixtape, ZIVA], systems to structure interaction between collaborators. These systems decompose work into tasks that can be handled individually by members. As such, they reduce the amount of task planning that teams need to do and lower the need for members to communicate with each other. Consequently, when tasks can be decomposed into independent fragments and members' roles can be well defined, these systems allow virtual teams thrive. When tasks can not be completely compartmentalized and members need to come together, interact, co-ideate, and deliberate, virtual teams are once again vulnerable to conflict and misunderstanding. 

\pranav{I have to bring up that we care about viability somewhere and this seemed like a good place}
Healthy team communication is foundational. A study found that while task-support interventions improved the performance of participant teams on average, interpersonal conflict in some teams negated the positive effects of the intervention~\cite{Bradley2003-aa}. Teams with healthy interpersonal processes provide a fertile ground for the positive impact of task-support interventions to improve performance further. Without effective communication, team performance can suffer and can even lead to teams not wanting to continue working together. Furthermore, team performance alone doesn't paint a complete picture of how a collaboration is going. Even high performing teams might have might have toxic culture, unresolved conflict, divisive interactions, burn out and high performance can be short lived. For a more holistic evaluation of a team, it is important to look beyond just \textit{team performance} and evaluate \textit{team viability}: the team's sustainability and capacity for continued success~\cite{Bell2011-rz,Cooperstein2017-cj, Whiting2019-wl}. Team viability is an emergent state that captures the potential of the team to continue performing well, the desire of the team to continue working together, and the extent to which the team can adapt to changing circumstances~\cite{Bell2011-rz}. Antecedents of team viability include perceived performance and interpersonal friction~\cite{Cooperstein2017-cj}. Consequently, viability requires that in addition to being performant, teams also have healthy communication and interpersonal processes in place~\cite{Cooperstein2017-cj}. 

\subsection{The right amount of team-friction: identifying interaction patterns of viable teams}
Research on what constitutes constructive team-communication patterns suggests that teams need to have the right amount of friction. Too much unresolved conflict and disregard for others' opinions and criticism can trigger negative emotions, causing members to get angry and distressed~\cite{Jung2015-px}. This can spiral out of control~\cite{Jung2015-px} and lead to a loss of viability. Too little disagreement and critical communication is also bad and could lower team performance, team satisfaction and consequently, viability. Open communication of ideas, suggestions, opinions, and issues, can help uncover new solutions~\cite{Menold2019-wc}, improve decision making \wesley{citation here as well?}, facilitate team learning~\cite{morrison2011speaking, Morrison2000-uu}, and help identify and address problems \wesley{citation here as well?}. However merely expressing opinions is not enough; to improve outcomes, team members must also engage with others' perspectives, foster inclusivity, and affirm each other~\cite{Salehi2018-vt, Carmeli2015-qv, Hoever2012-hn}. The diverse perspectives and unique expertise of individual members make teams potent and so, for teams to be effective it is crucial that team-members both speak up, expressing their perspectives, and that they listen to and engage with others' perspectives, in a respectful manner~\cite{morrison2011speaking}.

% A large body of work in organizational behavior has shown that positive relational dynamics are crucial for healthy functioning of teams~\cite{Lee2020-zn}. Respect, openness, connectedness, effective conflict management, and affect management can improve team creativity~\cite{Carmeli2015-qv}, resilience~\cite{Stephens2013-vx}, performance~\cite{Carmeli2015-qv,Edmondson1999-wl}, and ultimately, viability. Respectful interactions including engaging with the diverse perspectives of team members, ensuring inclusivity, and making sure people’s ideas and opinions are respected~\cite{Lee2020-zn} lead to higher cohesion and creativity~\cite{Carmeli2015-qv}. Teams with higher psychological safety and open communication place value on critical communication. Such open communication of disagreement and issues can lead to enhanced performance~\cite{Edmondson1999-wl} and decision making~\cite{Morrison2000-uu}. 

Researchers have developed methods to detect whether the interaction patterns in a team are healthy~\cite{Vrzakova2019-vk,Stewart2019-cs}. They have developed models that can leverage information about facial expression, eye gaze, head movements, speech, text, physiology, and interaction to detect the presence of positive traits~\cite{Cao2021-gm,Stewart2019-cs,Vrzakova2019-vk} such as turn-taking~\cite{Jokinen2013-ai}, interactivity~\cite{Ashenfelter2007-tk}, high-levels of empathy~\cite{Ishii2018-ex}, and team cohesion~\cite{Muller2018-ed}. These models have also enabled predicting team performance and team viability from a team’s interactions~\cite{Cao2021-gm}. While this line of work has furthered our understanding of which interpersonal processes and behaviors promote team viability, cultivating these prosocial behaviors in teams remains challenging~\cite{Lee2020-zn}. How do we translate these descriptive insights into prescriptive interventions? While we can use these insights to assemble effective teams by evaluating mutual compatibility of members, how can we help teams that have already been convened, develop positive communication patterns?

\subsection{Fostering constructive interaction patterns in teams}
Prior work has attributed the difficulty of establishing healthy communication to the low levels of information richness, lack of social cues, context, and shared emotion in computer-mediated teams~\cite{Hinds2003-ky}. In response, researchers have developed more information rich communication channels to improve social cues and emotional expression in these messaging systems~\cite{hassib2017heartchat}. This includes systems to communicate affect by altering the font and animation of text~\cite{buschek2015there,lee2006using,wang2004communicating}, via abstract visuals~\cite{viegas1999chat,tat2002visualising,tat2006crystalchat} and more recently, by using biosignals~\cite{hassib2017heartchat}. Researchers have also explored the design of computer-mediated interventions to nudge people towards more positive interaction patterns by providing them socio-metric feedback on group communication patterns~\cite{Leshed2007-up,Kim2012-jv,Leshed2009-eq,Tausczik2013-br}. 
% Some of these interventions and tools focus on providing feedback on teamwork practices as a mechanism to improve collaborative skills~\cite{He2017-xw,Leshed2007-up}. Researchers have built tools that automatically detect and provide sociometric feedback on group communication patterns~\cite{Kim2012-jv,Leshed2009-eq,Tausczik2013-br}.
% Chinmay's update: 
However, these systems have only had limited success, because they assume that highlighting problematic patterns is sufficient for teams to act on them and change their interaction norms. This is rarely seen to be the case in practice~\cite{He2017-xw,Leshed2007-up}. 
% Original: They highlight suboptimal group dynamics in an attempt to nudge teams to adopt more positive communication patterns. The positive effects of these systems have been limited because they make a simplifying assumption- highlighting problematic patterns is sufficient for teams to act on them and change their interaction norms. 

Some tools go beyond making extant behaviors salient and also make specific recommendations on how teams should alter their practices to move them closer to desired behaviors~\cite{Tausczik2013-br}. However, these systems don't capture true emotional states of teams- they only capture measurable proxies for underlying emotional states ( eg. synchronicity and positive sentiment in chat messages as a proxy for actual agreement between team members~\cite{Leshed2009-eq}). Since there is often a disconnect between how team members feel and what they are comfortable expressing~\cite{morrison2011speaking}, prescriptive interventions, based on measurable proxies, often fail to prompt team members to confront underlying issues and instead, team members game the system and merely seek to achieve desirable levels of surface-level proxies: prior work found that visualizing group-level agreement prompted team members to passively express agreement with each other while actually resulting in lower quality work~\cite{Leshed2009-eq}. This hints at teams adopting an avoidance approach to conflict resolution which leaves conflict unresolved and hinders teamwork~\cite{kankanhalli2006conflict}. 

Transforming and shaping interaction norms to promote open and respectful communication is challenging. It requires team members to take initiative and proactively engage in open and frank communication but team members often do not speak up. They may view expressing disagreement, voicing concerns, or asking questions as risky or they may believe that their inputs will not be taken seriously~\cite{morrison2011speaking} pushing them to avoid disagreeing entirely. These beliefs about speaking up are shaped by the interaction history of the team~\cite{morrison2011speaking}. For newly convened teams, an uncertainty about group norms and potential consequences of speaking up could discourage employees from speaking up. Relatedly, team members who do not strongly identify with their team or who are unsatisfied with their team, might think speaking up is futile~\cite{morrison2011speaking}. In such cases, a ``climate of silence''~\cite{Morrison2000-uu} becomes the norm which can undermine team performance and viability~\cite{perlow2003silence, argyris1991teaching}. 

\subsection{Psychological theories informing the design of our intervention}
To design an intervention to promote more constructive communication behaviors, we draw on organizational behavior theories around reorienting team norms and theories on empathy and perspective-taking. In designing our intervention, we draw on established mechanisms to regulate empathy and perspective-taking. To support the development of positive team dynamics via these regulatory mechanisms, we attempt to create an environment that is conducive to the emergence of new practices. We do this by borrowing on ``spaces'' which are analytical constructs studied in organizational psychology as bounded social setting that support the development of new interaction norms.

\subsubsection{Mechanisms to regulate perspective-taking}
A person's ability to take-perspectives is not an immutable trait~\cite{zaki2014empathy,curran2019understanding} and can be regulated by \textit{attention modulation}: drawing attention to others' emotions and affective states can increase perspective-taking~\cite{zaki2014empathy,curran2019understanding}. Perspective-taking is also regulated by \textit{appraisal} or an individual's evaluation of the authenticity and intensity of others' emotions~\cite{zaki2014empathy}. People might often choose to misrepresent their true emotions to adhere to social display rules and so, cues taken at face value might not accurately represent the target's true affective states~\cite{ansfield2007smiling,ekman1997smiles}. Enabling people to accurately appraise affective meaning of others' cues can improve perspective-taking. Taken together, this suggests the need for 1) communication channels that make people more attuned to others' affective states, 2) aids to augment people's ability to accurately assess others' affective states, and 3) interventions that lower the social and psychological barriers preventing people from expressing their true affective states.

\subsubsection{Spaces as enablers of change}


==> sections-old/02_relatedv3.tex <==
This research contributes to a growing body of work that aims to improve collaboration experiences of computer-mediated teams, tying together research in organizational behavior with research in HCI. We start by reviewing existing HCI research on software support for teams and highlight the need for systems that foster positive interaction norms. Drawing on research in organizational behavior, we attempt to characterize interaction patterns of performant and sustainable teams. We then look at how we can design effective interventions to cultivate these constructive interaction patterns in teams.     

\subsection{Beyond team assembly and task support: designing systems to nurture teams}
To improve outcomes of computer-mediated teams, human-computer interaction researchers have developed several systems aimed at assembling the right team for the task. Prior work has shown that teams composed of members with higher skill diversity~\cite{horwitz2007effects}, demographic diversity~\cite{lykourentzou2016personality}, and differing personality types~\cite{bear2011role} perform better and are more satisfied. Consequently, researchers have developed systems that optimize for these criteria and assemble teams with the most promise for success. Researchers have also built team-dating systems to improve collaboration by allowing people to experience work with different collaborators before team formation~\cite{Lykourentzou2017-yz}. Simultaneously, rotating members strategically can promote mixing of ideas~\cite{Salehi2018-vt}. To allow teams to cope with evolving work, researchers have also designed systems to on-board experts on-demand~\cite{Valentine2017-qu, Retelny2014-gk}. However, while these systems have demonstrated success in identifying good collaborators, team composition is naturally constrained by availability of talent. How can we help \textit{any} team achieve their full potential and work effectively?

One way to help computer-mediated teams work effectively is to provide support for task completion and coordination of effort. HCI researchers have designed several systems to support team tasks. This includes systems to create and manage workflows~\cite{Valentine2017-qu, rahman2020mixtape}, systems to structure interaction between collaborators~\cite{park2021facilitating, rahman2020mixtape}. These systems decompose work into tasks that can be handled individually by members. As such, they reduce the amount of task planning that teams need to do and lower the need for members to communicate with each other. Consequently, when tasks can be decomposed into independent fragments and members' roles can be well defined, these systems allow virtual teams thrive. When tasks can not be completely compartmentalized and members need to come together, interact, co-ideate, and deliberate, computer-mediated teams are once again vulnerable to conflict and misunderstanding~\cite{Whiting2019-wl, Whiting2020-pq}.

Healthy team communication is key to ensuring team viability. One prior study found that while task-support interventions improved the performance of participant teams on average, interpersonal conflict in some teams negated the positive effects of the intervention~\cite{Bradley2003-aa}. Teams with healthy interpersonal processes provide a fertile ground for the positive impact of task-support interventions to improve performance further. Without effective communication, team performance can suffer and can even lead to teams not wanting to continue working together. Furthermore, team performance alone doesn't paint a complete picture of how a collaboration is going. Even high performing teams might have might have toxic culture, unresolved conflict, divisive interactions, and member burnout. For a more holistic evaluation of a team, it is important to look beyond just \textit{team performance} and evaluate \textit{team viability}: the team's sustainability and capacity for continued success~\cite{Bell2011-rz,Cooperstein2017-cj, Whiting2019-wl}. Team viability is an emergent state that captures the potential of the team to continue performing well, the desire of the team to continue working together, and the extent to which the team can adapt to changing circumstances~\cite{Bell2011-rz}. Antecedents of team viability include perceived performance and interpersonal friction~\cite{Cooperstein2017-cj}. Consequently, viability requires that in addition to being performant, teams also have healthy communication and interpersonal processes in place~\cite{Cooperstein2017-cj}.

\subsection{The right amount of team-friction: identifying interaction patterns of viable teams}
% Interventions focused on improving interaction patterns in teams typically aim to improve positive exchanges in teams characterized by positive emotion and agreement~\cite{Tausczik2013-br}. However, research on what constitutes constructive team-communication patterns suggests that teams need to have the right amount of friction.
Research on what constitutes constructive team-communication patterns suggests that teams need to have the right amount of friction. Too much disagreement, unresolved conflict and disregard for others' opinions and criticism can trigger negative emotions, causing members to get angry and distressed~\cite{Jung2015-px}. This can spiral out of control~\cite{Jung2015-px} and lead to a loss of viability. Too little disagreement and critical communication is also bad and can impair team performance~\cite{perlow2003silence, argyris1991teaching}, team satisfaction and consequently, viability. Eliciting diverse perspectives by fostering open communication of ideas, opinions, and issues, can help uncover new solutions~\cite{Menold2019-wc}, improve decision making, facilitate team learning~\cite{morrison2011speaking, Morrison2000-uu}, and help identify problems. However, for teams to cultivate, and benefit from, this right amount of friction- where members communicate opinions openly but opinion conflicts don't hinder teams- they need ensure that members feel it is both \textit{safe} and \textit{effective} to voice their opinions~\cite{morrison2011speaking}. 

Team members feel \textit{safe} expressing themselves when they do not anticipate potential negative consequences of speaking up~\cite{morrison2011speaking}- they shouldn't be attacked or chastised for speaking up. However merely cultivating the safety necessary for people to express opinions is not enough; to improve outcomes, team members must also engage with others' perspectives, foster inclusivity, and affirm each other~\cite{Salehi2018-vt, Carmeli2015-qv, Hoever2012-hn}. This not only allows teams to incorporate diverse opinions of members but also signals to members that their opinions will be taken into account and acted upon. This can convince members that voicing their opinions is an \textit{effective} way to enact change and in turn motivates them continue to voice their opinions. The diverse perspectives and unique expertise of individual members make teams potent and so, for teams to be effective it is crucial that team-members both speak up, expressing their perspectives, and that they listen to and engage with others' perspectives, in a respectful manner~\cite{morrison2011speaking}.

% A large body of work in organizational behavior has shown that positive relational dynamics are crucial for healthy functioning of teams~\cite{Lee2020-zn}. Respect, openness, connectedness, effective conflict management, and affect management can improve team creativity~\cite{Carmeli2015-qv}, resilience~\cite{Stephens2013-vx}, performance~\cite{Carmeli2015-qv,Edmondson1999-wl}, and ultimately, viability. Respectful interactions including engaging with the diverse perspectives of team members, ensuring inclusivity, and making sure people’s ideas and opinions are respected~\cite{Lee2020-zn} lead to higher cohesion and creativity~\cite{Carmeli2015-qv}. Teams with higher psychological safety and open communication place value on critical communication. Such open communication of disagreement and issues can lead to enhanced performance~\cite{Edmondson1999-wl} and decision making~\cite{Morrison2000-uu}. 

HCI researchers have developed methods to detect whether the interaction patterns in a team are healthy~\cite{Vrzakova2019-vk,Stewart2019-cs}. They have developed models that can leverage information about facial expression, eye gaze, head movements, speech, text, physiology, and interaction to detect the presence of positive traits~\cite{Cao2021-gm,Stewart2019-cs,Vrzakova2019-vk} such as turn-taking~\cite{Jokinen2013-ai}, interactivity~\cite{Ashenfelter2007-tk}, high-levels of empathy~\cite{Ishii2018-ex}, and team cohesion~\cite{Muller2018-ed}. These models have also enabled predicting team performance and team viability from a team’s interactions~\cite{Cao2021-gm}. While this line of work has furthered our understanding of which interpersonal processes and behaviors promote team viability, cultivating these prosocial behaviors in teams remains challenging~\cite{Lee2020-zn}. Our work attempts to move from these descriptive insights towards prescriptive interventions to help teams develop positive communication patterns.  

\subsection{Fostering constructive interaction patterns in teams}
Prior work has attributed the difficulty of establishing healthy communication to the low levels of information richness, lack of social cues, context, and shared emotion in computer-mediated teams~\cite{Hinds2003-ky}. In response, researchers have developed more information rich communication channels to improve social cues and emotional expression in these messaging systems. This includes systems to communicate affect by altering the font and animation of text~\cite{buschek2015there,lee2006using,wang2004communicating}, and via abstract visuals~\cite{viegas1999chat,tat2002visualising,tat2006crystalchat}. Researchers have also explored the design of computer-mediated interventions to nudge people towards more positive interaction patterns by providing them socio-metric feedback on group communication patterns~\cite{Leshed2007-up,Kim2012-jv,Leshed2009-eq,Tausczik2013-br}. Some tools go beyond making extant behaviors salient and also make specific recommendations on how teams should alter their practices to move them closer to desired behaviors~\cite{Tausczik2013-br, kim2021moderator}. However, these systems have only had limited success, because they assume that highlighting problematic patterns and providing information-rich communication channels is sufficient to nudge team members to express their authentic opinions and change their interaction norms. In doing so, they ignore the social and psychological barriers preventing team members from speaking up: they do nothing to alter team members' perceived \textit{safety} and \textit{efficacy} of speaking up, necessary for open and healthy team communication. This can lead to undesirable outcomes: prior work found that visualizing group-level agreement led to a form of social loafing where team members expressed agreement with the majority opinion even if they did not agree with it with it and this ultimately resulted in lower quality work~\cite{Leshed2009-eq}.

Transforming and shaping interaction norms to promote open and respectful communication is challenging. It requires team members to take initiative and proactively engage in open and frank communication but team members often do not speak up. They may view expressing disagreement, voicing concerns, or asking questions as risky (low levels of perceived \textit{safety}) or they may believe that their inputs will not be taken seriously~\cite{morrison2011speaking} (low levels of perceived \textit{efficacy}) pushing them to avoid disagreeing entirely. These beliefs about speaking up are shaped by the interaction history of the team~\cite{morrison2011speaking}. For newly convened teams, an uncertainty about group norms and potential consequences of speaking up could lead to low perceived \textit{safety} and discourage employees from speaking up. Team members who do not strongly identify with their team, or who are unsatisfied with their team, might perceive low levels of \textit{efficacy} and think speaking up is futile~\cite{morrison2011speaking}. In such cases, a ``climate of silence''~\cite{Morrison2000-uu} becomes the norm which can undermine team performance and viability~\cite{perlow2003silence, argyris1991teaching}. 

\subsection{Psychological theories informing the design of our intervention}
To design an intervention to promote more constructive communication behaviors, we draw on perspective-taking as a useful tool to \textit{maintain} the \textit{safety} and \textit{efficacy} needed for healthy team communication. To support the \textit{development} of perspective-taking and positive team dynamics, we create an environment that is conducive to the emergence of new practices. We do this by creating a new ``space'' that provides a zone of \textit{safety} for experimental behaviors where teams can engage in a perspective-taking exercise.

\subsubsection{Inducing perspective-taking to maintain \textit{safety} and \textit{efficacy}}

Perspective-taking can be a useful tool to maintain perceived \textit{safety} of speaking up. By taking another’s perspective, team members are more likely to anticipate disagreement, recognizing that other people will have different views~\cite{Sessa1996-ba}. This can both reduce initial opposition to someone else's ideas as well as mentally prepare individuals to handle opposition to their ideas. Both of these together contribute to \textit{safety}.

Perspective-taking encompasses considering others’ evaluative standards which can lead to better evaluation of their ideas and more constructive feedback~\cite{Hoever2012-hn}. This can help team members feel heard and contribute to improved perceptions of \textit{efficacy}. Trying to understand someone else’s perspective can also trigger clarifying communication that can ultimately facilitate better understanding of everyone’s ideas~\cite{Hoever2012-hn}. Perspective-taking can lead to a cognitive reframing that leads to better integration of others’ ideas~\cite{Hargadon2006-ri}. Taken together, this suggests that perspective-taking can help teams take everyone's opinions into account and make everyone feel heard, both of which improve perceived \textit{efficacy} of speaking up.

\subsubsection{Creating an experimental space to induce perspective-taking} To suspend pre-existing interaction norms and induce perspective-taking, we draw on work that has explored the benefits of creating “spaces'' for transformative dialogue~\cite{Lee2020-zn, zietsma2010institutional}. Spaces are social settings separated by physical, temporal or symbolic boundaries from everyday work within which the salience of existing norms and interaction patterns diminishes. This creates an environment conducive to risky and counternormative behaviors that can catalyze the emergence of new dynamics~\cite{Lee2020-zn, bucher2016interplay, furnari2014interstitial, zietsma2010institutional}. Examples of such spaces include creating meetings to specifically engage in discussion about work challenges or organizing a retreat to help team members connect outside of work environments. Such “experimental spaces'' have been effective at reducing barriers to open communication in teams and consequently, fostering positive relational dynamics~\cite{Lee2020-zn}. We attempt to imagine what such a space might look like in the context of online team communication environments and how we might use such a space to induce perspective-taking towards the goal of improving team interactions.



==> sections-old/03_interventionv1.tex <==
To prompt team members to engage in perspective-taking, we designed and implemented \sys{}, a ``space'' embedded within a chat-based collaboration interface within which participants engage in a perspective-taking exercise. To explore different possible designs within a completely configurable chat environment, we built a custom chat-based collaboration environment (Figure \ref{fig:space}). This was a client-server web application built using Meteor.js. \sys{} attempts to improve team communication and perspective taking by providing an experimental space that encourages members to express their authentic emotions and prompts reflection on others' emotions. In doing so, \sys{} uses the power of ``spaces'' to facilitate counternormative behaviors. When triggered, \sys{} appears as a widget in the chat interface and disables the chat while teams carry out the perspective-taking exercise. The perspective-taking exercise (Figure \ref{fig:workflow}) in \sys{} was designed by drawing on known strategies to regulate perspective-taking.

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/intervention.pdf}
    \caption{\sys{} creates a separated space to within a team's chat within which members engage in a perspective-taking exercise. They A) share their own socio-emotional states, B) think about the socio-emotional states of their teammates and finally \sys{} presents them with C) a measure of the group’s cumulative socio-emotional state and D) a measure of how accurate they were at evaluating their teammates’ true socio-emotional states.}
    \label{fig:workflow}
\end{figure}

\subsection{Design of the perspective-taking exercise}
A person's ability to empathize or take-perspectives is not an immutable trait; instead it can be regulated by \textit{attention modulation}: drawing attention to others' emotions and affective states can increase perspective-taking~\cite{zaki2014empathy,curran2019understanding}. \sys{} prompts this process by asking each member to reflect on how other members might be feeling and by highlighting discrepancies between their evaluation of the group and the group's actual emotions. 

To aid reflection and discrepancy evaluation, while still maintaining the ambiguity and anonymity necessary to prompt authentic expression, \sys{} executes this process in three stages. First, \sys{} privately elicits how team members actually feel about working with their group (Figure \ref{fig:workflow}A) on a scale ranging from -5 to 5; -5 being the most negative and 5 the most positive.  Next, it asks each member, in private, to guess how each of the other members in the team might be feeling on the same scale, to nudge them to direct their attention towards others in the team (Figure \ref{fig:workflow}B). Finally, \sys{} calculates the mean of responses from the first stage to present each participant with feedback about the aggregate group climate, i.e. how positive/negative the group as a whole is feeling, without revealing individual responses (Figure \ref{fig:workflow}C). (While emotions i.e., how people feel, can be multi-faceted, we focus on a simple positive/negative model in our intervention to ease reflection and evaluation for participants.) Forcing reflection on others' emotions and presenting the average group climate are the first way \sys{} draws members' attention to the possibility that some team members might not be having a positive team experience. 

Beyond attention modulation, perspective-taking is also regulated by \textit{appraisal} or an individual's evaluation of the authenticity and intensity of others' emotions~\cite{zaki2014empathy}. Emotions expressed privately in the ``space'' are likely to be more authentic and uninhibited than those expressed in the chat. So, team members are more likely to recognize potential grievances and act on them when they are confronted with them within the space. Thus, to further aid in perspective-taking, \sys{} also presents every member with feedback on how accurate they were at guessing others' emotions (Figure \ref{fig:workflow}D) in their responses in the second stage above. Specifically, we use a  modified Krippendorff's alpha measure, such that for a team member $i$, the accuracy $\mathcal{A}_i$ is calculated as below, where $G_{ji}$ is $i$'s guess about $j$'s emotional state, and $S_j$ is $j$'s self-reported emotional state:
\begin{equation*}
    \mathcal{A}_i = max(0, 1 - \sum_{i,i\ne{}j}^n \frac{|G_{ji}-S_j|}{5(n-1)})
\end{equation*}

$\mathcal{A}_i$ is displayed to team member $i$ as a percentage for easier interpretation. This accuracy measure is at 100\% if a member guessed all other members emotions perfectly, and at 0\% (in expectation) for random guesses. Krippendorff's alpha can be negative (when disagreements exceed what can be expected by chance) but this is not useful for our reflective purposes, so we show participants 0\% accuracy at minimum.
% would mean the average of the differences was more than $5$, i.e. the member guessed the . 
By controlling for agreements by random chance, this measure emphasizes discrepancies between an individual's evaluation of others' emotions and their actual emotions, with the goal of drawing attention to the valence and arousal levels of others' emotions.
